Beyond Kalman Filters: Deep Learning-Based Filters for Improved Object Tracking

Traditional tracking-by-detection systems typically employ Kalman filters (KF) for state estimation. However, the KF requires domain-specific design choices and it is ill-suited to handling non-linear motion patterns. To address these limitations, we propose two innovative data-driven filtering methods. Our first method employs a Bayesian filter with a trainable motion model to predict an object's future location and combines its predictions with observations gained from an object detector to enhance bounding box prediction accuracy. Moreover, it dispenses with most domain-specific design choices characteristic of the KF. The second method, an end-to-end trainable filter, goes a step further by learning to correct detector errors, further minimizing the need for domain expertise. Additionally, we introduce a range of motion model architectures based on Recurrent Neural Networks, Neural Ordinary Differential Equations, and Conditional Neural Processes, that are combined with the proposed filtering methods. Our extensive evaluation across multiple datasets demonstrates that our proposed filters outperform the traditional KF in object tracking, especially in the case of non-linear motion patterns -- the use case our filters are best suited to. We also conduct noise robustness analysis of our filters with convincing positive results. We further propose a new cost function for associating observations with tracks. Our tracker, which incorporates this new association cost with our proposed filters, outperforms the conventional SORT method and other motion-based trackers in multi-object tracking according to multiple metrics on motion-rich DanceTrack and SportsMOT datasets.

==> backup.tex <==
\section{Bayesian Update of a Normal Distribution}
\label{appendix:bayesian_updates}

In this section, we present the derivation of mean and covariance matrix parameter updates when the Bayes's rule is applied. We only consider the case with a single observation, which suffices for our purposes. The derivation for multiple observations can be found in \cite{gaussian_product}. In Section \ref{appendix:univariate_bayesian_updates}, we perform the derivation for univariate Gaussian distributions, and in Section \ref{appendix:multivariate_bayesian_updates}, we perform the derivation for multivariate Gaussian distributions.

\subsection{Univariate Normal Distribution}
\label{appendix:univariate_bayesian_updates}

We aim to derive the mean $\tilde{\mu}$ and $\tilde{\sigma}$ of the posterior distribution $f_{x|D} \sim \mathcal{N}(\tilde{\mu}, \tilde{\sigma})$ as defined by Bayes's rule, where the posterior distribution is proportional to the product of the prior $f_x \sim \mathcal{N}(\hat{\mu}, \hat{\sigma})$ and the likelihood $f_{D|x} \sim \mathcal{N}(\mu, \sigma)$, i.e., $f_{x|D} \propto f_x \cdot f_{D_x}$. Hence, we only need to derive the parameters of the scaled Gaussian PDF $f_x (y) \cdot f_{D|x} (y) = C \cdot f_{x|D} (y) = C \cdot \frac{1}{\sqrt{2\pi\tilde{\sigma}^2}} e^{-\frac{(y-\tilde{\mu})^2}{2\tilde{\sigma}^2}}$, where $C$ is a constant. Derivation is as follows:
%
\begin{align}
f_x (y) \cdot f_{D|x} (y) &= \frac{1}{\sqrt{2\pi\hat{\sigma}^2}} e^{-\frac{(y-\hat{\mu})^2}{2\hat{\sigma}^2}} \cdot \frac{1}{\sqrt{2\pi\sigma^2}} e^{-\frac{(y-\mu)^2}{2\sigma^2}} \\
&= \frac{1}{2\pi\hat{\sigma}\sigma} e^{-\frac{1}{2}(\frac{(y-\hat{\mu})^2}{\hat{\sigma}^2} -\frac{(y-\mu)^2}{\sigma^2})}
\end{align}
%
We define $\alpha(y) = \frac{(y-\hat{\mu})^2}{\hat{\sigma}^2} -\frac{(y-\mu)^2}{\sigma^2}$, with the goal of restructuring it in a form like $\alpha(y) = \frac{(y-\tilde{\mu})^2}{\tilde{\sigma}^2} + C$, where $C$ is a constant:
%
\begin{align}
\alpha(y) &= \frac{y^2-2y\hat{\mu}+\hat{\mu}^2}{\hat{\sigma}^2} - \frac{y^2-2y\mu+\mu^2}{\sigma^2} 
\\
&= y^2 (\frac{1}{\hat{\sigma}^2} + \frac{1}{\sigma^2}) - 2y(\frac{\hat{\mu}}{\hat{\sigma}^2} + \frac{\mu}{\sigma^2})
+ (\frac{\hat{\mu}^2}{\hat{\sigma}^2} + \frac{\mu^2}{\sigma^2}) \\
&= y^2 (\frac{\sigma^2 + \hat{\sigma}^2}{\sigma^2\hat{\sigma}^2}) - 2y\frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2\hat{\sigma}^2}
+ \frac{\sigma^2\hat{\mu}^2 + \hat{\sigma}^2\mu^2}{\sigma^2\hat{\sigma}^2} \\
&= \frac{\sigma^2 + \hat{\sigma}^2}{\sigma^2\hat{\sigma}^2} \left(y^2- 2y\frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2}
+ \frac{\sigma^2\hat{\mu}^2 + \hat{\sigma}^2\mu^2}{\sigma^2 + \hat{\sigma}^2} \right) \\
&= \frac{\sigma^2 + \hat{\sigma}^2}{\sigma^2\hat{\sigma}^2} \left(y^2- 2y\frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2}
+ \left(\frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2}\right)^2 - \left(\frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2}\right)^2 + \frac{\sigma^2\hat{\mu}^2 + \hat{\sigma}^2\mu^2}{\sigma^2 + \hat{\sigma}^2} \right) \\
&= \frac{\sigma^2 + \hat{\sigma}^2}{\sigma^2\hat{\sigma}^2} \left(y - \frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2}\right)^2 + C \\
&= \frac{(\tilde{y}-\tilde{\mu})^2}{\tilde{\sigma}^2} + C \label{eq:univariate_final_form}
\end{align}
%
From this we can conclude that: 
%
\begin{align}
\tilde{\sigma}^2 = \frac{\sigma^2\hat{\sigma}^2}{\sigma^2 + \hat{\sigma}^2} = \frac{1}{\frac{1}{\hat{\sigma}^2} + \frac{1}{\sigma^2}}
\end{align}
%
If we use Gaussian PDF \textit{precision} denoted as $p = \frac{1}{\sigma^2}$ instead of variance, we get a nicer form:
%
\begin{align}
\tilde{p} = \hat{p} + p
\end{align}
%
From Eq.\ \eqref{eq:univariate_final_form} we can also conclude that:
%
\begin{align}
\tilde{\mu} = \frac{\sigma^2\hat{\mu} + \hat{\sigma}^2\mu}{\sigma^2 + \hat{\sigma}^2} = \frac{\frac{\mu}{\sigma^2} + \frac{\hat{\mu}}{\hat{\sigma}^2}}{\frac{1}{\sigma^2} + \frac{1}{\hat{\sigma}^2}} = \frac{p\cdot\mu + \hat{p}\cdot\hat{\mu}}{p + \hat{p}}
\end{align}
%
Finally, we have the scaled posterior PDF:
%
\begin{align}
f_x (y) \cdot f_{D|x} (y) &= \frac{1}{2\pi\hat{\sigma}^2\sigma^2} e^{\frac{(\tilde{y}-\tilde{\mu})^2}{\tilde{\sigma}^2} + C} \\ 
&= \frac{1}{\sqrt{2\pi\tilde{\sigma}^2}} e^{\frac{(\tilde{y}-\tilde{\mu})^2}{\tilde{\sigma}^2}} \cdot C \\
&= f_{x|D} \cdot C
\end{align}
%
The derivation for the multivariate normal distribution in the next section is analogous to this one. Note that in the case of independent variables, i.e., a diagonal covariance matrix, applying Bayes's rule updates for a univariate normal distribution per variable is sufficient.

\subsection{Multivariate Normal Distribution}
\label{appendix:multivariate_bayesian_updates}

Again, we only need to derive the parameters of the scaled Gaussian PDF $f_x (y) \cdot f_{D|x} (y) = C \cdot f_{x|D} (y) = C \cdot \frac{1}{\sqrt{(2\pi)^{k}|\tilde{\Sigma}|^2}} e^{-\frac{1}{2}(y-\tilde{\mu})^{^\top}\tilde{\Sigma}^{-1}(y-\tilde{\mu})}$, where $C$ is a constant. Derivation is as follows:
%
\begin{align}
f_x (y) \cdot f_{D|x} (y) &= \frac{1}{\sqrt{(2\pi)^{k}|\hat{\Sigma}|^2}} e^{-\frac{1}{2}(y-\hat{\mu})^{^\top}\hat{\Sigma}^{-1}(y-\hat{\mu})} \cdot \frac{1}{\sqrt{(2\pi)^{k}|\Sigma|^2}} e^{-\frac{1}{2}(y-\mu)^{^\top}\Sigma^{-1}(y-\mu)} \\
&= \frac{1}{(2\pi)^{k}|\hat{\Sigma}||\Sigma|} e^{-\frac{1}{2}\left((y-\hat{\mu})^{^\top}\hat{\Sigma}^{-1}(y-\hat{\mu}) + (y-\mu)^{^\top}\Sigma^{-1}(y-\mu)\right)}
\end{align}
%
We define $\beta(y) = (y-\hat{\mu})^{^\top}\hat{\Sigma}^{-1}(y-\hat{\mu}) + (y-\mu)^{^\top}\Sigma^{-1}(y-\mu)$, with the goal of restructuring it in a form like $\beta(y) = (y-\tilde{\mu})^{^\top}\tilde{\Sigma}^{-1}(y-\tilde{\mu}) + C = y^{^\top}\tilde{\Sigma}^{-1}y - y^{^\top}\tilde{\Sigma}^{-1}\tilde{\mu} - \tilde{\mu}^{^\top}\tilde{\Sigma}^{-1}y + \tilde{\mu}^{^\top}\tilde{\Sigma}^{-1}\tilde{\mu} + C$, where $C$ is a constant:
%
\begin{align}
\beta(y) &= y^{^\top}\hat{\Sigma}^{-1}y - y^{^\top}\hat{\Sigma}^{-1}\hat{\mu} - \hat{\mu}^{^\top}\hat{\Sigma}^{-1}y + \hat{\mu}^{^\top}\hat{\Sigma}^{-1}\hat{\mu}
+ y^{^\top}\Sigma^{-1}y - y^{^\top}\Sigma^{-1}\mu - \mu^{^\top}\Sigma^{-1}y + \mu^{^\top}\Sigma^{-1}\mu \\
&= y^{^\top}\left(\hat{\Sigma}^{-1} + \Sigma^{-1}\right)y - y^{^\top}\left(\hat{\Sigma}^{-1}\hat{\mu} + \Sigma^{-1}\mu\right) - \left(\hat{\mu}^{^\top}\hat{\Sigma}^{-1} + \mu^{^\top}\Sigma^{-1}\right)y + \hat{\mu}^{^\top}\hat{\Sigma}^{-1}\hat{\mu} + \mu^{^\top}\Sigma^{-1}\mu
\end{align}
%
By examining the first element in the addition in Eq. (20), we can hypothesize that $\tilde{\Sigma}^{-1} = \hat{\Sigma}^{-1} + \Sigma^{-1}$. Given that the first element is already in this form, we only need to demonstrate that it aligns with the second ($- y^{^\top}\tilde{\Sigma}^{-1}\tilde{\mu}$) and third ($- \tilde{\mu}^{^\top}\tilde{\Sigma}^{-1}y$) elements of the addition, under the same assumption. Any remaining terms are considered part of the constant. The negative of the second element in the addition is:
%
\begin{align}
y^{^\top}\left(\hat{\Sigma}^{-1}\hat{\mu} + \Sigma^{-1}\mu\right) &= y^{^\top}\tilde{\Sigma}^{-1}\tilde{\Sigma}\left(\hat{\Sigma}^{-1}\hat{\mu} + \Sigma^{-1}\mu\right) \\
&= y^{^\top}\tilde{\Sigma}^{-1}\tilde{\mu}
\end{align}
%
where we hypothesize $\tilde{\mu} = \tilde{\Sigma}\left(\hat{\Sigma}^{-1}\hat{\mu} + \Sigma^{-1}\mu\right) = \tilde{\Sigma}\hat{\Sigma}^{-1}\hat{\mu} + \tilde{\Sigma}\Sigma^{-1}\mu$. The negative of the third element in the addition is:
%
\begin{align}
\left(\hat{\mu}^{^\top}\hat{\Sigma}^{-1} + \mu^{^\top}\Sigma^{-1}\right)y &= \left(\hat{\mu}^{^\top}\hat{\Sigma}^{-1} + \mu^{^\top}\Sigma^{-1}\right)\tilde{\Sigma}\tilde{\Sigma}^{-1}y \\
&= \left(\tilde{\Sigma}\left(\hat{\mu}^{^\top}\hat{\Sigma}^{-1} + \mu^{^\top}\Sigma^{-1}\right)^{^\top}\right)^{^\top}\tilde{\Sigma}^{-1}y \\
&= \left(\tilde{\Sigma}\left(\hat{\Sigma}^{-1}\hat{\mu} + \Sigma^{-1}\mu\right)\right)^{^\top}\tilde{\Sigma}^{-1}y \\
&= \tilde{\mu}^{^\top}\tilde{\Sigma}^{-1}y
\end{align}
%
which proves our hypothesis using the fact that transpose of a symmetric covariance matrix is the same matrix. Parameters of the scaled posterior PDF are as follows:
%
\begin{align}
\tilde{\Sigma}^{-1} = \hat{\Sigma}^{-1} + \Sigma^{-1}
\end{align}
%
\begin{align}
\tilde{\mu} = \tilde{\Sigma}\hat{\Sigma}^{-1}\hat{\mu} + \tilde{\Sigma}\Sigma^{-1}\mu
\end{align}
%

